A global-local approach for hydraulic phase-field fracture in poroelastic media

In this work, phase-field modeling of hydraulic fractures in porous media is extended towards a global-local approach. Therein, the failure behavior is solely analyzed in a (small) local domain. In the surrounding medium, a simplified and linearized system of equations is solved. Both domains are coupled by Robin-type interface conditions. The fracture(s) inside the local domain are allowed to propagate and consequently both subdomains change within time. Here, a predictor-corrector strategy is adopted in which the local domain is dynamically adjusted to the current fracture pattern. The resulting framework is algorithmically described in detail and substantiated with some numerical tests.

==> sec4.tex <==
%=======================================================================
\sectpa[Section4]{Different Global-Local Scenarios}
%=======================================================================

We assume the Global-Local formulation is at the converged state, which is denoted as $(\bm u_{G,n},\bm u_{L,n},d_{L,n}$
$,\bm u_{\Gamma,n},\bm\lambda_{C,n},\bm\lambda_{L,n})$. The
Global-Local approach is augmented by a {\it dynamic allocation} of a local state using an adaptive scheme which has to be performed at
time step $t_{n}$. By the adaptivity procedure, we  mean: ({a}) to
determine which global elements need to be refined and identified by
$\calB^{\;adapt}_G\subset\calB_G$; ({b}) to create the new fictitious
domain $\calB^{\;new}_F:=\calB^{\;old}_F\cup\calB^{\;adapt}_F$ with $\calB^{\;adapt}_F:= \calB^{\;adapt}_G$ and as a result
a new local domain is defined as $\calB^{\;new}_L:=\calB^{\;old}_L\cup\calB^{\;adapt}_L$, see Fig. \ref{adapt}; ({c}) to determine a new local interface denoted as $\Gamma_L$;
({d}) to interpolate the old global solution in $\calB^{\;adapt}_L$. {All these steps refer to predictor steps. 
The corrector step is explained in Section \ref{Section4_a2}.}
{We briefly notice that the principal idea of this adaptive scheme 
is inspired from \cite{Wick15Adapt} in which a predictor-corrector scheme for 
mesh refinement in the crack zone was proposed.}
 
%=======================================================================
\sectpb[Section4_a1]{Predictor step}
{In this section, we start explaining the predictor step.}
\begin{itemize}
 	\item {\em \textbf{Determining global elements which have to be refined}}		
\end{itemize}
Recall that the {interfaces} at the global, fictitious and local domains are denoted by $\Gamma_G \subset \calB_G$, $\Gamma_F \subset \calB_F$ and $\Gamma_L \subset \calB_L$. We denote $e_{G}\in\calB_G$, $e_{F}\in\calB_F$ and $e_{L}\in\calB_L$ as the elements in the global, fictitious and local domain. Let $E^1_{G,i}, E^2_{G,i}, E^3_{G,i}$ and $E^4_{G,i}$ refer to the left, top, right and bottom global edges for the $i^{th}$ element $e_{G,i}$, respectively (because, it is quadrilateral hence it has four edges). Accordingly, $E^q_{F,i}\in e_{F,i}$ and $E^q_{L,i}\in e_{L,i}$ with $\;q=(1,2,3,4)$ refer to the fictitious and local edges, see Fig. \ref{adapt}.  

%Doing so, we find nodal value $\bm x_L\in\Gamma_L$ on the local interface such that, its crack phase-field has a less value compared to the given threshold value denoted as $\texttt{TOL}_{d}$. Afterwards, the local edge $E^{k}_{L,i}\in\Gamma_L$ has to be find such that ${\bm x_L}\in E^{k}_{L,i}$. We then find the corresponding fictitious edge $E^{k}_{F,i}$ that is a coarse projection of the local edge. Knowing that, $E^{k}_{G,i}:=E^{k}_{F,i}$, we finally determine all global element that shares the same edge. If this global elements are not allready within $\calB_F$ then this element has to be refined. 

We now develop a procedure, to determine the global elements $e_{G,i}$
which have at least one edge $E^{q}_{G,i}$ such that their fine resolution at the
local level, i.e. $E^{q}_{L,i}$, reaches to the crack phase-field threshold
value. Thus $e_{G,i}$ has to be refined. The predictor step for
the adaptive scheme of the Global-Local formulation {is explained} in Algorithm \ref{alg_1}.

\begin{algorithm}[H]\small
	\caption{\em Predictor step for the adaptive procedure.}	
	\label{alg_1}
	Let $0<\texttt{TOL}_{d}<1$ be given. For the $d_L:=d_{L,n}\;\in\calB_L$, 
find corresponding $e_{G}\in\calB_G$ which {must be} refined using the following steps:
	\begin{enumerate}
		\item Find $\bm x_L\in\Gamma_L$ such that $d_L({\bm
	x}_L)<\texttt{TOL}_{d}$ on $\Gamma_L$:\\[2mm] 
{\it Checking criterion:} If "\texttt{Yes}" proceed {to step 2.}
If "\texttt{No}" stop,
		\item find $E^{q}_{L,i}\in\Gamma_L$ such that ${\bm x_L}\in E^{q}_{L,i}$,
		\item find $E^{q}_{G,i}=\calP^{-1}E^{q}_{L,i}$ (corresponding edge {in} $\calB_G$),
		\item find $e_{G}\in\calB_G$ and $e_{G}\not\in\calB_F$ such that $E^{q}_{G,i}\in e_{G}$.
    \end{enumerate}
\end{algorithm}

Here, $\calP:\Gamma_G\rightarrow\Gamma_L$ is denoted as a projection/geometrical operator which maps the global to the local interface by $E^{q}_{L,i}:=\calP E^{q}_{G,i}$. 

\begin{itemize}
	\item {\em \textbf{Creating new fictitious and local domains: $(\calB^{\;new}_F,\calB^{\;new}_L)$}}		
\end{itemize}
We are now able to determine a new fictitious and local domains. Knowing $e_{G}$ from the previous step, the new fictitious domain is $\calB^{\;new}_F:=\calB^{\;old}_F\cup\calB^{\;adapt}_F$ such that $\calB^{\;adapt}_F:=e_{G}$. As a result, a new local domain is $\calB^{\;new}_L:=\calB^{\;old}_L\cup\calB^{\;adapt}_L$ such that $\calB^{\;adapt}_L$ is a fine discretization (including heterogeneity as well) of $\calB^{\;adapt}_F$, see Fig. \ref{adapt}.
\begin{itemize}
	\item {\em \textbf{Determining the coupling interface: $(\Gamma_G,\;\Gamma_F,\;\Gamma_L)$}}		
\end{itemize}
{So far, we have identified {\it new} fictitious and local domains. Next, we determine $\Gamma_F\subset\calB_F$, due to its coarse discretization. Afterwards, we find the local interface $\Gamma_L \subset \calB_L$ by projecting $\Gamma_F$ to $\calB_L$. Finally, it is trivial that $\Gamma_G:=\Gamma_F$, because $\calB_F$ and $\calB_G$ are in the same discretization space. 

The edge $E^q_{F,i}\in\Gamma_F$ is on the interface if 
\begin{equation}\label{inter1}
E^{q}_{F,i}\in\Gamma_F \;\; \mbox{if} \;\;\nexists \;\;i,j\;:E^{q}_{F,i}=E^{r}_{F,j} ,\quad \mbox{for}\;q,r=(1,2,3,4),
\end{equation}
{which} means if an edge $E^q_{F,i}$ is shared between two elements in $\calB_F$, it is not on the interface (inner edge) and if it belongs only to one element, 
then {it must also} belong to interface (outer edge). As a result, we define the fictitious interface as $\Gamma_F = \substackrel{i,q}{{\huge \texttt{A}}} \, E^{q}_{F,i}$, hence $\Gamma_L = \substackrel{i,k}{{\huge \texttt{A}}} \, E^{q}_{L,i}$ with $ E^{q}_{L,i}:=\calP E^{q}_{F,i}$. 
\begin{itemize}
	\item {\em \textbf{Interpolating the old solution at $t^n$ {from
	the global to the local mesh}}}		
\end{itemize}
Given a continuous function $\bm u^{adapt}_G$ that is $\bm u_G$ in $\calB^{\;adapt}_G$, we define the linear interpolation operator  $\mathcal{\pi}:\calB^{\;adapt}_G\rightarrow\calB^{\;adapt}_L$ to $\bm u^{adapt}_G$ by
\begin{equation}\label{inter3}
{\bm u^{adapt}_{L,n}}(\bm{x}):=\mathcal{\pi}{\bm u^{adapt}_{G,n}}=\bm N_u^G(\bm{x}){\hat{\bm u}^{adapt}_{G,n}}\quad\mbox{for}\;\; {\bm{x}}\in\calB^{\;adapt}_L. 
\end{equation}
where $\bm N_u^G(x)$ is defined in Appendix A. Hence, ${\bm u^{new}_{L,n}}:={\bm u_{L,n}}\cup{\bm u^{adapt}_{L,n}}$.


%=======================================================================
\sectpb[Section4_a2]{{Corrector step}}

%\begin{itemize}
%	\item {\em \textbf{Corrector step for adaptive scheme at $t^n$}}		
%\end{itemize}

 
We introduce a corrector step {in which the computation is rerun on the newly determined local mesh.} To this end, we compute Global-Local
solutions until {the} checking criterion in Algorithm \ref{alg_1} is not
satisfied (\texttt{No}). 
That means we could not find additional local edges on the interface such that $d_L({\bm x}_L)<\texttt{TOL}_{d}$ on $\Gamma_L$ holds.

{Let us write Algorithm \ref{TableGL} in} the following abstract form
\begin{equation}\label{inter4}
{\bm s_n}=\texttt{GL}({\bm s_{n-1}}),
\end{equation}
with ${\bm s}=(\bm u_{G},\bm u_{L},d_{L},\bm u_{\Gamma},\bm\lambda_{C},\bm\lambda_{L})$. We define an intermediate solution ${\bm s^{j}_{n-1}}$ at fixed $t^{n}$ such that the corrector step for adaptive scheme reads,
\begin{equation}\label{inter5}
{\bm s^{j}_{n-1}}=\texttt{GL}({\bm s_{n-1}}). 
\end{equation}
Perform Algorithm \ref{alg_1}, if the \textit{checking criterion} in step 1 is
satisfied. But, if this is not the case, then the corrector step is fulfilled, thus set ${\bm
s^{j}_{n-1}}=:{\bm s_{n}}$ and stop; else $j+1\rightarrow j$. 


%=======================================================================
\sectpb[Section4_a3]{{The final predictor-corrector scheme}}

The aforementioned predictor-corrector adaptivity procedure is summarized in Algorithm \ref{alg_2} as follows,
\begin{algorithm}[H]\small
	\caption{\em Predictor-corrector steps for the adaptive procedure.}
	\label{alg_2}
	Let $0<\texttt{TOL}_{d}<1$ be given. For the $d_L:=d_{L,n}\;\in\calB_L$, find corresponding $e_{G}\in\calB_G$ which have to be refined using the following steps:
	\begin{enumerate}
		\item Compute the intermediate solution by ${\bm s^{j}_{n-1}}=\texttt{GL}({\bm s_{n-1}})$,
		\item perform Algorithm \ref{alg_1} if \textit{Checking criterion} is satisfied (\texttt{Yes}),
		\item if \textit{checking criterion} in Algorithm \ref{alg_1} is not satisfied, then the corrector step is fulfilled, thus set ${\bm s^{j}_{n-1}}=:{\bm s_{n}}$ and stop; else $j+1\rightarrow j$.
	\end{enumerate}
%
\end{algorithm}	
Fig. \ref{adapt} depicts one iteration of the predictor-corrector steps for the adaptive procedure which is illustrated in Algorithm \ref{alg_2}.
\begin{figure}[!ht]
	\centering
	{\includegraphics[clip,trim=0cm 3cm 0cm 4.5cm, width=14cm]{Figures/adapt1.pdf}}  %left, bottom, right and top 
	\caption{{Explanation of the predictor-corrector adaptive scheme.}
	}
	\label{adapt}
\end{figure}

We notice that for the brutal fracture behavior, where a complete
failure {happens} in one load increment, 
Algorithm \ref{alg_2} has an important effect. This is mainly because the corrector step is performed until there is no nodal point on the interface such that $d_L({\bm x}_L)<\texttt{TOL}_{d}$ holds. If this is fulfilled, the adaptivity procedure stops and goes to the next load increment. Thus brutal fracture can be observed in the next time step. This is illustrated in the numerical example of the Section \ref{Section522}. 

The performance of Algorithm \ref{alg_1} and Algorithm \ref{alg_2} is depicted in Fig. \ref{A1} and Fig. \ref{A2}. This example refers to the isotropic single-edge notch under tension. The numerical setup is given in \cite{MieWelHof10b}. By applying predictor-corrector steps, we will have a more regularized fracture surface. This is observed for instance in Fig. \ref{A2} step 58, step 60 and step 62 (right figures). But that is not the case, if we only apply predictor step. For instance in Fig. \ref{A1}, at step 58, after the predictor step (in the absence of the corrector stage). Here we do not have a regularized fracture surface. It will be regularized in the next load increment which is shown in step 59 . That is also observed in steps 60 and 63 in Fig. \ref{A1}, as well. To compare these effects on the global level, we refer to the load-displacement curve in Fig. \ref{B4}a. It was observed that the corrector procedure applied to the predictor step improved the Global-Local results.

\begin{figure}[!ht]
	\centering
	{\includegraphics[clip,trim=0cm 9cm 0cm 10cm, width=16cm]{Figures/A1.pdf}}  %left, bottom, right and top 
	\caption{Global-Local approach augmented with the predictor adaptive scheme given in Algorithm \ref{alg_1}; Fracture of isotropic single-edge-notched plate under tension per loading steps.
	}
	\label{A1}
\end{figure}

\begin{figure}[!ht]
	\centering
	{\includegraphics[clip,trim=0cm 9cm 0cm 8.8cm, width=16cm]{Figures/A2.pdf}}  %left, bottom, right and top 
	\caption{Global-Local approach augmented with the predictor-corrector adaptive scheme indicated in Algorithm \ref{alg_2}; Fracture of isotropic single-edge-notched plate under tension per loading steps.
	}
	\label{A2}
\end{figure}

%=======================================================================
\sectpb[Section4_homoPhF]{Homogenized {phase-field solution on the global level}}
%=======================================================================
We determine the coarse representation of the crack phase-field. Here we denote $(\bm u_{G,n},\bm u_{L,n},d_{L,n}$
$,\bm u_{\Gamma,n},\bm\lambda_{C,n},\bm\lambda_{L,n})$ to be the converged solution of the Global-Local approach. We emphasis that the computation of the global phase-field $d_G$ is a post-processing step. The \textit{homogenized global crack phase-field} solution can be determine based on the following ways.

(\textit{a}) \textbf{Global crack phase-field solution.} We solve the crack phase-field given in (\ref{eq282}) after having obtained the converged global solution by
\begin{equation}\label{global_crack1}
	d_G =\substackrel{d_G \in W }{\mbox{argmin}} \,
	[-g^{\prime}({d_{G+})\calH(\bm u_{G,n};\BM_G) - l_G \delta_d.\gamma_l}],
\end{equation}
with,
\begin{equation}\label{global_crack2}
l_G := l_L \frac{h_G}{h_L}\quad \mbox{and}\quad\BM_G := \BM_L. 
\end{equation}
where $\calH$ is described by (\ref{eq29_H3}) and formulated on the global level. The last condition in (\ref{global_crack2})$_2$ holds because we assumed the structural tensor at the global level inclined with identical angle as the local level. This holds in the case of the transverse isotropic setting.

(\textit{b}) \textbf{Homogeneous crack phase-field solution.} Assume that at the global level the transition zone of the crack phase-field vanishes. That results in a free isotropic and anisotropic Laplacian operator $\Delta (\bullet)=0$ in (\ref{eq282}). Hence, the second and third terms in (\ref{eq29_H5}) become zero. Following that Eq. \ref{eq282} at the quasi-static stationery state is restated by  
\begin{equation}\label{homo_phf_sol}
d_G=\frac{1}{1+2(1-\kappa)\calH(\bm u_{G,n};\BM_G)} \;\in[0,1],
\end{equation}
{such} that if $\calH\rightarrow\infty \;\mbox{then}\;d_G=0$ and for $\calH\rightarrow 0  \;\mbox{then}\;d_G=1$ holds. The homogeneous crack phase-field solution $d_G$ in (\ref{homo_phf_sol}) is independent of the $l_G$ but the global crack phase-field solution in (\ref{global_crack1}) depends on $l_G$.
At the global level we do not have any given imperfection (e.g. notch shaped). That is located \textit{only} at the local level. However, (\ref{global_crack1}) or (\ref{homo_phf_sol}) still provides the desired crack direction because of $\calH(\bm u_{G,n};\BM_G)$. This is due to the fact that $\bm u_{G,n}$ is determined based on the given $\bm u_\Gamma^{k,\frac{1}{2}}$ which is upscaled from local level, see (\ref{Coupl6nG}). As a result, the crack driving force at the global level is the \textit{true projection} of the constitutive non-linearity at the local level. That is varitionally consistent and resulting from the upscaling procedure (i.e. information which is transformed from the local level to the global scale). 


%+++++++++++++++++++++++++++
%
%The related counterparts of the standard fourth-order elasticity tensor $\mathbb{C}$ read in this case
%\begin{equation}\label{eff_elast1}
%\texttt{Voigt:}\;\;\mathbb{C}_G:=\frac{1}{|\calB_L|}\int_{\calB_L}{\mathbb{C}_L},\quad\texttt{Reuss:}\;\;\mathbb{C}_G:=\big(\frac{1}{|\calB_L|}\int_{\calB_L}{\mathbb{C}^{-1}_L}\big)^{-1}
%\end{equation}
%
%we further assume,
%
%\begin{equation}\label{eff_elast2}
%l_G = l_L \frac{h_G}{h_L},\quad \BM_L = \BM_G.
%\end{equation}
%
%
%++++++++++++++++++++++++++

